Low-rank updates of matrix functions

We consider the task of updating a matrix function $f(A)$ when the matrix $A\in{\mathbb C}^{n \times n}$ is subject to a low-rank modification. In other words, we aim at approximating $f(A+D)-f(A)$ for a matrix $D$ of rank $k \ll n$. The approach proposed in this paper attains efficiency by projecting onto tensorized Krylov subspaces produced by matrix-vector multiplications with $A$ and $A^*$. We prove the approximations obtained from $m$ steps of the proposed methods are exact if $f$ is a polynomial of degree at most $m$ and use this as a basis for proving a variety of convergence results, in particular for the matrix exponential and for Markov functions. We illustrate the performance of our method by considering various examples from network analysis, where our approach can be used to cheaply update centrality and communicability measures.

==> decay.tex <==
\section{Decay properties of the update matrix}\label{sec:decay}

In many important applications, see also Section~\ref{sec:experiments}, the vectors $\vb,\vc$ are (multiples of) canonical unit vectors or linear combinations of a few consecutive canonical unit vectors. In these situations, one typically observes a rapid decay of the update matrix $f(A+\vb\vb^\ast)-f(A)$ for entries far away from the nonzero pattern of $\vb\vc^\ast$. This is tightly linked to well-known decay properties of the matrix inverse~\cite{Demko1977,DemkoMossSmith1984}. Decay bounds for matrix functions are typically derived for banded matrices with small bandwidths. Motivated by the application of up-/down-dating communicability measures in graphs, discussed in Section~\ref{sec:experiments}, we formulate the decay bounds using the more general concept of distance in the graph corresponding to $A$; see also~\cite[Section 5 \& 7]{BenziSimoncini2015}.

For a Hermitian matrix $A \in \Rnn$, the corresponding (undirected) graph $G_A = (V_A,E_A)$ is defined by
\begin{equation}\label{eq:graph}
V_A = \{1,\dots,n\} \text{ and } E_A = \{ \{i,j\} : a_{ij} \neq 0\}.
\end{equation}
The \emph{distance} $\distA(i,j)$ between two nodes $i,j \in V_A$ is defined as the length of the shortest path in $G$ which connects $i$ and $j$. Without loss of generality, we assume in the following that $G_A$ is \emph{connected}, so that $\distA(i,j) < \infty$ for all $i$ and $j$. As $G_A$ is undirected, $\distA(i,j) = \distA(j,i)$.

The following classical theorem on decay in the matrix inverse will be the basis of our analysis in this section. While originally stated for banded matrices, we reformulate it in terms of the graph distance.

\begin{theorem}[Theorem 2.4 in~\cite{DemkoMossSmith1984}]\label{the:decay_demko}
Let $A \in \Cnn$ be Hermitian positive definite, with smallest and largest eigenvalue $\lmin(A)$ and $\lmax(A)$ and Euclidean norm condition number $\kappa(A)$. Then 
\begin{equation}\label{eq:demko_bound}
|[A^{-1}]_{i,j} | \leq C_Aq_A^{\distA(i,j)} 
\end{equation}
with 
\begin{equation}\label{eq:decay_factor}
 q_A=\frac{\sqrt{\kappa(A)}-1}{\sqrt{\kappa(A)}+1}
\mbox{ and }
 C_A=\max \left \{ \frac 1{\lambda_{\min}(A)}, \frac{\big(1+\sqrt{\kappa(A)}\big)^2}{2\lambda_{\max}(A) }\right \}.
\end{equation}
\end{theorem}

The result of Theorem~\ref{the:decay_demko}---when applied to shifted versions of $A$---directly implies a result for the decay in the update matrix $f(A+\vb\vc^\ast)f(A)$ when $A$ is Hermitian positive definite, $\vb,\vc$ are unit vectors and $f$ is a Stieltjes function.

\begin{theorem}\label{the:decay_stieltjes}
Let $A \in \Cnn$ be Hermitian positive definite, let $f$ be a Stieltjes function, assume that $f(A + \ve_k\ve_\ell^\ast)$ is defined and let
$$F = f(A+\ve_k\ve_\ell^\ast)-f(A)$$
Then the entries of $F$ can be bounded as
\begin{equation}\label{eq:decay_update}
|F_{i,j}| \leq \frac{4 |f'(\lmin(A))|}{K} q_A^{\distA(i,k)+\distA(\ell,j)}
\end{equation}
where $C_A$ and $q_A$ are defined in~\eqref{eq:decay_factor} and
$$K = \min_{t \geq 0} \{|1 + \ve_\ell^\ast(A+tI)^{-1}\ve_k|\} > 0.$$
\end{theorem}
\begin{proof}
Using the representation for $F$ by the \SMW formula again, we have
\begin{eqnarray}
|F_{i,j}| &=& |\ve_i^\ast(f(A+\ve_k\ve_\ell^\ast)-f(A))\ve_j| \nonumber\\
					&\leq& \int_0^\infty \frac{1}{|1 + \ve_\ell(A+tI)^{-1}\ve_k^\ast|} \cdot |\ve_i^\ast (A+tI)^{-1} \ve_k| \cdot |\ve_j^\ast (A+tI)^{-1} \ve_\ell| \dmu \nonumber\\
					&\leq& \frac{1}{K} \int_0^\infty |[(A+tI)^{-1}]_{i,k}| \cdot |[(A+tI)^{-1}]_{\ell,j}| \dmu\label{eq:decay_stieltjes_proof1}
\end{eqnarray}
Note that $K > 0$ when $f(A+\ve_k\ve_\ell^\ast$ is defined, as all shifted matrices $A+tI\ve_k\ve_\ell^\ast$ must be invertible. Applying the result of Theorem~\ref{the:decay_demko} to the entries of $(A+tI)^{-1}$ in~\eqref{eq:decay_stieltjes_proof1} then yields
\begin{equation}\label{eq:decay_stieltjes_proof2}
|F_{i,j}| \leq \frac{1}{K} \int_0^\infty C_A^2 q_{A+tI}^{\distA(i,k)}\cdot q_{A+tI}^{\distA(\ell,j)}\dmu
\end{equation}
Noting that $C_{A+tI} \leq 2/(\lmin(A) + t)$, see also~\cite{FrommerSchimmelSchweitzer2017} and that $q_{A+tI} \leq q_A$ for all $t \geq 0$, we find
\begin{equation}\label{eq:decay_stieltjes_proof3}
|F_{i,j}| \leq \frac{1}{K} q_A^{\distA(i,k)+\distA(\ell,j)} \int_0^\infty \frac{4}{(\lmin(A)+t)^2}\dmu
\end{equation}
Using~\eqref{eq:f_prime} then completes the proof.
\end{proof}

\begin{figure}
\begin{center}
\includegraphics[width=.65\textwidth]{figs/decay.pdf}
\end{center}
\caption{Decay pattern on a logarithmic scale of $f(A + \ve_{201}\ve_{200}^H) - f(A)$, where $A = \tridiag(-1,3,-1) \in \R^{400 \times 400}$ and $f(z) = z^{-1/2}$.\label{fig:decay_tridiag}}
\end{figure}

From~\eqref{eq:decay_update}, it is immediately obvious that the entries of $F_{i,j}$ become small as soon as \emph{either} $\distA(i,j)$ \emph{or} $\distA(j,\ell)$ is large, with especially rapid decay when both distances are large at the same time. We illustrate this by a simple example. 

\begin{example}\label{ex:decay}
Consider the tridiagonal matrix $A = \tridiag(-1,3,-1) \!\in\! \R^{400 \times 400}$, the function $f(z) = z^{-1/2}$ and $\vu = \ve_{201},\vv = \ve_{200}$. Figure~\ref{fig:decay_tridiag} shows the magnitude of the entries of $F$, and we observe that the entries decay rapidly away from the position at which the modification was performed (for the graph of a tridiagonal matrix $A$ we have $\distA(i,j) = |i-j|$) exactly as predicted by Theorem~\ref{the:decay_stieltjes}. In particular, note that all entries of the update matrix that are larger than, e.g., $10^{-10}$ in magnitude, are located inside a submatrix of size about $40 \times 40$.
\end{example}

The decay behavior predicted by Theorem~\ref{the:decay_stieltjes} and illustrated in Example~\ref{ex:decay} is very useful also from a computational point of view, as it means that the computations for approximating the update matrix need not be performed on the whole matrix, but only on a smaller submatrix, depending on the accuracy one wants to reach. Of course, this requires that the bound~\eqref{eq:decay_update} can be evaluated, which means that, e.g., certain spectral information of $A$ must be available.

\comment{Repeat this for exponential/Cauchy integral formula?}
